What Right-Angle Corners Reveal About an Uncalibrated Camera: Convex Cones, Certified Bounds and Identifiability

The corner of a box or a room, where three perpendicular edges meet, appears in an image as three segments meeting at a point. We ask what such junctions reveal about an uncalibrated camera's intrinsic parameters. Each junction is consistent with an explicit convex set of cameras; when only the focal length is unknown, this set is an interval in closed form. These sets are computed from the image alone, so calibrating from many junctions is a convex feasibility problem. Almost every junction bounds the focal length from below; we characterize when one also bounds it from above, and when many junctions determine it exactly. For a known vertex, the bounds can be certified against any bounded error in the measured edge directions.

==> latexmkrc <==
# Lets supplement.tex read the article's numbering (package xr): when the
# supplement is compiled, latexmk first compiles main.tex to produce main.aux.
add_cus_dep('tex', 'aux', 0, 'makeexternaldocument');
sub makeexternaldocument {
    if (!($root_filename eq $_[0])) {
        system("latexmk -cd -pdf \"$_[0]\"");
    }
}

